Convergence Analysis of Gradient EM for Multi-component Gaussian Mixture

In this paper, we study convergence properties of the gradient Expectation-Maximization algorithm \cite{lange1995gradient} for Gaussian Mixture Models for general number of clusters and mixing coefficients. We derive the convergence rate depending on the mixing coefficients, minimum and maximum pairwise distances between the true centers and dimensionality and number of components; and obtain a near-optimal local contraction radius. While there have been some recent notable works that derive local convergence rates for EM in the two equal mixture symmetric GMM, in the more general case, the derivations need structurally different and non-trivial arguments. We use recent tools from learning theory and empirical processes to achieve our theoretical results.

==> ming_add_a.tex <==
\bas{
& \max\left\{ c\sqrt{\log( c_1\frac{M^2\kappa}{\pi_{\min}} +2\log \left(2\rmax+\min\{d,M\}\right)}, \right.\\
\sqrt{\min\{d,M\}}\max\{c_2\sqrt{\log (\rmin/4)_+},8\sqrt{3}\}\right\} \\
\leq & \max \{ c \sqrt{\log(c_1\frac{M^2\kappa}{\pi_{\min}}+c_2\rmax+c_3{\min\{d,M\}})}, \\
c'\sqrt{\min\{d,M\}}\max\{\sqrt{\log(\rmax+e)}\}\}\\
\leq & O(\sqrt{\min\{d,M\}}\sqrt{\log(\max(\frac{M^2\kappa}{\pi_{\min}},\rmax,\min\{d,M\}))})
}


==> r_to_infty.tex <==
\begin{lemma}
Consider the Gaussian mixture model with 3 equal weight clusters, whose means are $\bmu_1^*, \bmu_2^*, \bmu_3^*$ respectively, and covariance $\sigma^2I$. Let $\eta = \frac{1}{\sigma^2}$ and $\sigma$ is small enough such that $\|\bmu_i^*-\bmu_i\|^2-\|\bmu_i^*-\bmu_j\|^2 \le -(2+\eta)\sigma^2 r^2, \forall j\ne i$, then
\bas{
 \nabla_{\bmu_i}Q(\bmu|\bmu) \to  \bmu_i^*-\bmu_i , \quad \forall i =1,2,3.
}
as $\sigma \to 0$.
\end{lemma}
\begin{proof}
\ba{
&\nabla_{\bmu_1}Q(\bmu|\bmu)  = \bE_X\left[ w_1(X)(X-\bmu_1) \right] \nonumber\\
=& \frac{1}{3}\bE_{X\sim \cN(\bmu_1^*,\sigma^2I)}\left[ w_1(X)(X-\bmu_1) \right]+\frac{1}{3}\bE_{X\sim \cN(\bmu_2^*,\sigma^2I)}\left[ w_1(X)(X-\bmu_1) \right]+\frac{1}{3}\bE_{X\sim \cN(\bmu_3^*,\sigma^2I)}\left[ w_1(X)(X-\bmu_1) \right] \label{eq:three_mixture}
}
Now we look at each term separately. First define the difference in distances as 
\bas{
\alpha_{ij}(X) = \|X-\bmu_i\|^2-\|X-\bmu_j\|^2, \forall i,j\in [3]
}
For $X\sim \cN(\bmu_1^*,\sigma^2I)$, define $\cE_1=\{X: \|X-\bmu_1^*\|\le \sigma r \}$, %$\alpha_{1i}(X) = \|X-\bmu_1\|^2-\|X-\bmu_i\|^2, \forall i\ne 1$. 
 From triangle inequality we have
\bas{
\alpha_{1i}(X) \le& \|X-\bmu_1^*\|^2+\|\bmu_1^*-\bmu_1\|^2+\|X-\bmu_1^*\|^2-\|\bmu_1^*-\bmu_i\|^2\\
\le& 2\sigma^2 r^2+(\|\bmu_1^*-\bmu_1\|^2-\|\bmu_1^*-\bmu_i\|^2),\quad \forall X\in \cE_1\\
\le & -\eta\sigma^2 r^2, \mbox{ if } \|\bmu_1^*-\bmu_1\|^2-\|\bmu_1^*-\bmu_i\|^2 \le -(2+\eta)\sigma^2 r^2
}
Note $\frac{1}{\sigma^2}\|X-\bmu_1^*\|^2\sim \chi^2_d$, by the tail bound of $\chi^2$ distribution \cite{laurent2000adaptive},
\ba{
P(X\in \cE_1^c) \le \sigma e^{-\frac{(r-\sqrt{d})^2}{2}}
\label{eq:prob_e1c}
}
Then we can simplify the weight function as 
\bas{
w_1(X) =& \frac{\exp\left(-\frac{(X-\bmu_1)^T(X-\bmu_1)}{2\sigma^2}\right)}{\sum_{j\ne 1}\exp\left(-\frac{(X-\bmu_j)^T(X-\bmu_j)}{2\sigma^2}\right)}\\
=& \frac{1}{1+\sum_{j\ne 1} \exp \left( \frac{\alpha_{1j}(X)}{2\sigma^2} \right)}
}
Therefore by law of total expectation,
\bas{
&\bE_{X\sim \cN(\bmu_1^*,\sigma^2I)}\left[ w_1(X)(X-\bmu_1) \right]\\
=&\bE_{X\sim \cN(\bmu_1^*,\sigma^2I)}\left[ X-\bmu_1 \right]-\bE_{X\sim \cN(\bmu_1^*,\sigma^2I)}\left[ (1-w_1(X))(X-\bmu_1) \right]\\
=& \bmu_1^*-\bmu_1-\bE_{X\sim \cN(\bmu_1^*,\sigma^2I)}\left[ (1-w_1(X))(X-\bmu_1)|\cE_1 \right]P(\cE_1)-\bE_{X\sim \cN(\bmu_1^*,\sigma^2I)}\left[ (1-w_1(X))(X-\bmu_1) |\cE_1^c \right]P(\cE_1^c)
}
We want to bound the norm of the expectation terms.
\bas{
&\|\bE_{X\sim \cN(\bmu_1^*,\sigma^2I)}\left[ (1-w_1(X))(X-\bmu_1)|\cE_1 \right]P(\cE_1)\|\\
=& \| \bE_{X\sim \cN(\bmu_1^*,\sigma^2I)}\left[ \frac{\sum_{j\ne 1} \exp \left( \frac{\alpha_{1j}(X)}{2\sigma^2} \right)}{1+\sum_{j\ne 1} \exp \left( \frac{\alpha_{1j}(X)}{2\sigma^2} \right)}(X-\bmu_1)|\cE_1 \right]P(\cE_1) \| \\
\le & P(\cE_1) \| \sum_{j\ne 1}  \bE_{X\sim \cN(\bmu_1^*,\sigma^2I)}\left[ \exp \left( \frac{\alpha_{1j}(X)}{2\sigma^2} \right) (X-\bmu_1)|\cE_1 \right] \| \\
\le & 2\|\bmu_1^*-\bmu_1\|  \exp \left( -\frac{\eta r^2}{2} \right) P(\cE_1)  \le  2\|\bmu_1^*-\bmu_1\|  \exp \left( -\frac{\eta r^2}{2} \right)
}
For the other term,
\bas{
&\| \bE_{X\sim \cN(\bmu_1^*,\sigma^2I)}\left[ (1-w_1(X))(X-\bmu_1) |\cE_1^c \right]P(\cE_1^c) \| \\
\le & \| \bE_{X\sim \cN(\bmu_1^*,\sigma^2I)}\left[ X-\bmu_1 |\cE_1^c \right]P(\cE_1^c)\| \\
\le & \|\bE_{X\sim \cN(\bmu_1^*,\sigma^2I)}\left[ X-\bmu_1^* |\cE_1^c \right]P(\cE_1^c)\|+\|\bmu_1^*-\bmu_1\| P(\cE_1^c)\\
\le & \bE_{X\sim \cN(\bmu_1^*,\sigma^2I)}\| X-\bmu_1^*\|+\|\bmu_1^*-\bmu_1\| P(\cE_1^c)\\
=& \sigma \frac{\sqrt{2}\Gamma\left(\frac{d+1}{2}\right)}{\Gamma\left(\frac{d}{2}\right)}+\|\bmu_1^*-\bmu_1\| P(\cE_1^c)\\
\le & \sigma \left(\frac{\sqrt{2}\Gamma\left(\frac{d+1}{2}\right)}{\Gamma\left(\frac{d}{2}\right)}+\|\bmu_1^*-\bmu_1\| \exp(-\frac{(r-\sqrt{d})^2}{2})\right)
}
The last inequality comes from \eqref{eq:prob_e1c},
Therefore for $r\ge \sqrt{d}$, %as $\sigma\to 0, \eta\to \infty$, 
\beq{
\bsplt{
&\| \bE_{X\sim \cN(\bmu_1^*,\sigma^2I)}\left[ w_1(X)(X-\bmu_1) \right] -(  \bmu_1^*-\bmu_1)\| \\
\le & \exp(-\eta r^2/2)\|\bmu_1^*-\bmu_1\|+ \sigma \left(\frac{\sqrt{2}\Gamma\left(\frac{d+1}{2}\right)}{\Gamma\left(\frac{d}{2}\right)}+\|\bmu_1^*-\bmu_1\| \exp(-\frac{(r-\sqrt{d})^2}{2})\right)
}
\label{eq:grad_mu1_1}
}
% E_2
Similarly, define $\cE_2=\{ X\sim \cN(\bmu_2^*,\sigma^2I): \|X-\bmu_2^*\|\le \sigma r \}$, by assumption we know for $X\in \cE_2$, $\alpha_{2i}(X) \le -\eta\sigma^2r^2, \forall i\ne 2$.
\beq{
\bsplt{
& \| \bE_{X\sim \cN(\bmu_2^*,\sigma^2I)}\left[ w_1(X)(X-\bmu_1) \right] \| \\
=& \| \bE_{X\sim \cN(\bmu_2^*,\sigma^2I)}\left[ w_1(X)(X-\bmu_1)|\cE_2 \right]P(\cE_2)+\bE_{X\sim \cN(\bmu_2^*,\sigma^2I)}\left[ w_1(X)(X-\bmu_1) |\cE_2^c \right]P(\cE_2^c) \| \\
\le & \exp(-\eta r^2)\|\bmu_2^*-\bmu_1\|+ \bE_{X\sim \cN(\bmu_2^*,\sigma^2I)} \|X-\bmu_2^*\| +\|\bmu_2^*-\bmu_1\|P(\cE_2^c)\\
\le & \exp(-\eta r^2/2)\|\bmu_2^*-\bmu_1\|+ \sigma \left(\frac{\sqrt{2}\Gamma\left(\frac{d+1}{2}\right)}{\Gamma\left(\frac{d}{2}\right)}+\|\bmu_2^*-\bmu_1\| \exp(-\frac{(r-\sqrt{d})^2}{2})\right)
}
\label{eq:grad_mu1_2}
}
And 
\beq{
\bsplt{
& \| \bE_{X\sim \cN(\bmu_3^*,\sigma^2I)}\left[ w_1(X)(X-\bmu_1) \right] \| \\
\le & \exp(-\eta r^2/2)\|\bmu_3^*-\bmu_1\|+ \sigma \left(\frac{\sqrt{2}\Gamma\left(\frac{d+1}{2}\right)}{\Gamma\left(\frac{d}{2}\right)}+\|\bmu_3^*-\bmu_1\| \exp(-\frac{(r-\sqrt{d})^2}{2})\right)
}
\label{eq:grad_mu1_3}
}
Plug \eqref{eq:grad_mu1_1}, \eqref{eq:grad_mu1_2}, \eqref{eq:grad_mu1_3} back to \eqref{eq:three_mixture},
\bas{
&\| \nabla_{\bmu_1}\cL(\bmu) - ( \bmu_1^*-\bmu_1)\| \\
\le & \exp(-\eta r^2/2)\frac{1}{3}\sum_{i=1}^3 \|\bmu_i^*-\bmu_1\| + \sigma \left(\frac{3\sqrt{2}\Gamma\left(\frac{d+1}{2}\right)}{\Gamma\left(\frac{d}{2}\right)}+\frac{1}{3}\sum_{i=1}^3 \|\bmu_i^*-\bmu_1\| \exp(-\frac{(r-\sqrt{d})^2}{2})\right)\\
&=\frac{1}{3}\sum_{i=1}^3 \|\bmu_i^*-\bmu_1\| \left(  \exp(-\eta r^2/2)+\sigma  \exp(-\frac{(r-\sqrt{d})^2}{2}) \right)+ \frac{3\sigma\sqrt{2}\Gamma\left(\frac{d+1}{2}\right)}{\Gamma\left(\frac{d}{2}\right)} \to 0
}
as $\sigma \to 0$.
\end{proof}

==> second_taylor.tex <==
\begin{proof}[Proof of Theorem \ref{th:gmm_gs}]
Consider the difference of the gradient corresponding to $\bmu_i$, without loss of generality, assume $i=1$.
\beq{
\bsplt{
\nabla Q(\bmu_1^t|\bmu_1^t) - \nabla q(\bmu_1^t)  = &  \bE w_1(X;\bmu_1^t)(X-\bmu_1^t) -  \bE w_1(X;\bmu_1^*)(X-\bmu_1^t)\\
=&  \bE (w_1(X;\bmu_1^t) -w_1(X;\bmu_1^*))(X-\bmu_1^*)+\bE (w_1(X;\bmu_1^t) -w_1(X;\bmu_1^*))(\bmu_1^*-\bmu_1^t) 
}
\label{eq:gs_lhs_step1}
}
For any given $X$, expanding the difference of weights around $\bmu_1^*$ we have
\beq{
\bsplt{
w_1(X;\bmu_1^t) -w_1(X;\bmu_1^*) =&  w_1(X;\bmu^*) (1-w_1(X;\bmu^*) )(X-\bmu_1^*)^T(\bmu_1^t-\bmu_1^*)\\
&- w_1(X;\bmu^*) w_2(X;\bmu^*) (X-\bmu_2^*)^T(\bmu_2^t-\bmu_2^*)\\
&- w_1(X;\bmu^*) w_3(X;\bmu^*) (X-\bmu_3^*)^T(\bmu_3^t-\bmu_3^*)\\
&+\frac{1}{2}(\bmu^t-\bmu^*)^T\nabla^2 w_1(X;\bmu^\xi)(\bmu^t-\bmu^*)
}
\label{eq:diff_w1}
}
The $\nabla^2 w_1(X;\bmu_1^\xi)$ is the Hessian of $w_1$ with respect to $\bmu^*$ evaluated at some point $\bmu^\xi \in \bB(\bmu_1^*, \|\bmu_1^t-\bmu_1^*\|) \times \bB(\bmu_2^*, \|\bmu_2^t-\bmu_2^*\|) \times \bB(\bmu_3^*, \|\bmu_3^t-\bmu_3^*\|)$.

Plugging \eqref{eq:diff_w1} into \eqref{eq:gs_lhs_step1} we have, \bowei{add in other terms}
\bas{
\nabla Q(\bmu_1^t|\bmu_1^t) - \nabla q(\bmu_1^t)  = & \bE (w_1(X;\bmu_1^*) (1-w_1(X;\bmu_1^*) )(X-\bmu_1^*)^T(\bmu_1^t-\bmu_1^*))(X-\bmu_1^*)\\
&+\bE (w_1(X;\bmu_1^*) (1-w_1(X;\bmu_1^*) )(X-\bmu_1^*)^T(\bmu_1^t-\bmu_1^*))(\bmu_1^*-\bmu_1^t) \\
&+ \bE \frac{1}{2}(\bmu_1^t-\bmu_1^*)^T\nabla^2 w_1(X;\bmu_1^\xi)(\bmu_1^t-\bmu_1^*) (X-\bmu_1^t)\\
:=& A+B+C
}
\paragraph{Bounding $A$} 
\input{mingzhang_a}

\paragraph{Bounding $B$}
Expanding $B$ based on the mixtures, we have
\bas{
\|B\| \le& \frac{1}{12}\bE_{X\sim \cN_1} \|X-\bmu_1^*\| \|\bmu_1^t-\bmu_1^*\|^2+ \frac{1}{3}\bE_{X\sim \cN_2} (w_1(X;\bmu_1^*) (1-w_1(X;\bmu_1^*) )\|X-\bmu_1^*\| \|\bmu_1^t-\bmu_1^*\|^2 \\
&+ \frac{1}{3}\bE_{X\sim \cN_3} (w_1(X;\bmu_1^*) (1-w_1(X;\bmu_1^*) )\|X-\bmu_1^*\| \|\bmu_1^t-\bmu_1^*\|^2\\
\frac{\|B\| }{\|\bmu_1^t-\bmu_1^*\|^2} \le & \frac{1}{12} \cdot \frac{\sqrt{2}\Gamma\left( \frac{d+1}{2}\right)}{\Gamma\left( \frac{d}{2}\right)} + \frac{2}{3}\bE_{X\sim \cN_2} (w_1(X;\bmu_1^*) \|X-\bmu_1^*\|\\
\le & \frac{1}{12} \cdot \frac{\sqrt{2}\Gamma\left( \frac{d+1}{2}\right)}{\Gamma\left( \frac{d}{2}\right)} + \frac{2}{3}\int_X \frac{\phi(X;\bmu_1^*)\phi(X;\bmu_2^*)}{\phi(X;\bmu_1^*)+\phi(X;\bmu_2^*)+\phi(X;\bmu_3^*)} \|X-\bmu_1^*\| dx\\
\le &  \frac{1}{12} \cdot \frac{\sqrt{2}\Gamma\left( \frac{d+1}{2}\right)}{\Gamma\left( \frac{d}{2}\right)} + \frac{2}{3}\int_X \phi_1(X;\bmu_1^*) \|X-\bmu_1^*\| dx\\
=& \frac{3\sqrt{2}\Gamma\left( \frac{d+1}{2}\right)}{4\Gamma\left( \frac{d}{2}\right)} 
}

\paragraph{Bounding $C$}
First note the Hessian of $w_1$ can be written as
\beq{
\bsplt{
\nabla^2_{\bmu_1} w_1(X;\bmu_1) =& \nabla_{\bmu_1} w_1(X;\bmu_1) (1-w_1(X;\bmu_1) )(X-\bmu_1)^T\\
=& -w_1(X;\bmu_1) (1-w_1(X;\bmu_1) ) I_d+w_1(X;\bmu_1) (1-w_1(X;\bmu_1) )(1-2w_1(X;\bmu_1))(X-\bmu_1)(X-\bmu_1)^T
}
\label{eq:hessian_w1}
}
Plugging \eqref{eq:hessian_w1} to $C$ we have,
\bas{
C = &  \frac{1}{2} \bE(\bmu_1^t-\bmu_1^*)^T \left( -w_1(X;\bmu_1^\xi) (1-w_1(X;\bmu_1^\xi) ) I_d \right) (\bmu_1^t-\bmu_1^*) (X-\bmu_1^t)\\
&+\frac{1}{2} \bE(\bmu_1^t-\bmu_1^*)^T \left( w_1(X;\bmu_1^\xi) (1-w_1(X;\bmu_1^\xi) )(1-2w_1(X;\bmu_1^\xi))(X-\bmu_1^\xi)(X-\bmu_1^\xi)^T \right) (\bmu_1^t-\bmu_1^*) (X-\bmu_1^t)\\
\|C\| =& \frac{ \|\bmu_1^t-\bmu_1^*\|^2}{2} \bE \left( -w_1(X;\bmu_1^\xi) (1-w_1(X;\bmu_1^\xi) )  \right) \|X-\bmu_1^t\|\\
&+\frac{ \|\bmu_1^t-\bmu_1^*\|^2}{2} \bE \left( w_1(X;\bmu_1^\xi) (1-w_1(X;\bmu_1^\xi) )|1-2w_1(X;\bmu_1^\xi)|\|(X-\bmu_1^\xi)(X-\bmu_1^\xi)^T\|_{op} \right) \|X-\bmu_1^t\|\\
\frac{\|C\|}{\|\bmu_1^t-\bmu_1^*\|^2}\le & \frac{1}{2}\bE \left( w_1(X;\bmu_1^\xi)  \right) (\|X-\bmu_1^\xi\|+a)+\frac{1}{2}\bE \left( w_1(X;\bmu_1^\xi) (\|X-\bmu_1^\xi\|^3+ a\|X-\bmu_1^\xi\|^2\right) 
}

\end{proof}
